N-body Networks: a Covariant Hierarchical Neural Network Architecture for Learning Atomic Potentials

We describe N-body networks, a neural network architecture for learning the behavior and properties of complex many body physical systems. Our specific application is to learn atomic potential energy surfaces for use in molecular dynamics simulations. Our architecture is novel in that (a) it is based on a hierarchical decomposition of the many body system into subsytems, (b) the activations of the network correspond to the internal state of each subsystem, (c) the "neurons" in the network are constructed explicitly so as to guarantee that each of the activations is covariant to rotations, (d) the neurons operate entirely in Fourier space, and the nonlinearities are realized by tensor products followed by Clebsch-Gordan decompositions. As part of the description of our network, we give a characterization of what way the weights of the network may interact with the activations so as to ensure that the covariance property is maintained.

==> CCN.tex <==
\section{Covariant compositional networks}

==> aggregation.tex <==
\subsection{Covariant aggregation functions} 

Definitions \ref{def: cnm} and \ref{def: mbnn} lay down the general architecture of the networks that we use 
to model Physical systems. 
What remains to define are the \m{\Phi_i} aggregation functions 
%To satisfy the covariance property, however 
%It remains to define the aggragation function \m{\Phi} 
that relate subsytems at different levels. %, while ensuring that the network satisfies covariance.  
In general, \m{\Phi_i} will be of a form similar to \rf{eq: classical aggregation}, in that it involves 
(a) accumulating contributions from each of the children of the given node, 
(b) weighting the different contributions by some learnt weight matrices, 
(c) applying a pointwise nonlinearity to the result. 
What makes the situation more complex than in classical neural nets is that \m{\Phi_i} has two different 
types of arguments which interact with each other: 
the \m{\phi_j} state vectors and \m{\V r_j} position vectors. 
Moreover, to satisfy (CM4), \m{\Phi_i(\V r_{\ch_1},\ldots,\V r_{\ch_k},\phi_{\ch_1}\ldots,\phi_{\ch_k})} must be 
\begin{compactenum}[~~1.]
\item \emph{Covariant} to the simultaneous action of \m{G} on each of its arguments. % in order to satisfy (CM4). 
%\m{\V r_{\ch_1},\ldots,\V r_{\ch_k},\phi_{\ch_1}\ldots,\phi_{\ch_k}}.  
%on in the sense of (CM4). 
\item \emph{Invariant} with respect to permutations of \m{\cbrN{\sseq{\ch}{k}}}, since this ordering is arbitrary.
\end{compactenum}
\smallskip

\noindent 
A key observation is that by virtue of \m{\Omega} being a vector space that 
\m{G} acts on, \m{\Omega} itself is a representation space of \m{G}.  %corresponding to some 
We will denote the corresponding representation \m{\rho_\Omega}. 
For example, when \m{\Omega=\RR^3} and \m{G} is the group of three-dimensional rotations, 
for any rotation \m{g\tin G}, letting \m{\rho_\Omega(g)\tin\RR^{3\times 3}}  
be the corresponding rotation matrix, 
any \m{\V r\tin \RR^3} transforms under \m{g} as \m{\V r\mapsto \rho_\Omega(g)\ts \V r}. 

As a generalization, given a collection of vectors \m{\cbrN{\V r_j}_{j=1}^m}, their mean, 
or \emph{first order moment},   
\[T^{(1)}=\ovr{m} \sum_{j=1}^{m} \V r_j,\] 
also transforms under \m{G} as \m{T^{(1)} \mapsto \rho_\Omega(g)\cdot  T^{(1)}}. 
The \emph{second order moment matrix} 
\[T^{(2)}=\ovr{m} \sum_{j=1}^{m} \V r_j\otimes \V r_j\]
transforms as \m{T^{(2)}\mapsto \rho_\Omega(g)\cdot  T^{(2)}\cdot (\rho_\Omega(g))^\top}. 
In general, the \m{k}\emph{'th order moment tensor}  
\begin{equation}\label{eq: moment tensor}
T^{(k)}=\ovr{m} \sum_{i=1}^{m}\: \underbrace{\V r_i\otimes \V r_i \otimes \ldots \otimes \V r_i}_{k\textrm{ times}}
\end{equation} 
transforms as 
\[T^{(k)}_{\sseq{i}{k}}\mapsto [\rho_\Omega(g)]_{i_1}{}^{\!\!i'_1}\, [\rho_\Omega(g)]_{i_2}{}^{\!\!i'_2}\, 
\ldots \, [\rho_\Omega(g)]_{i_k}{}^{\!\!i'_k}\; T^{(k)}_{\sseq{i'}{k}},\]
where we have used the Einstein convention for summing over repeated indices. 
Moreover, these equations are not specific to just rotations. 
It is generally the case that if \m{\sseq{\V r}{m}} are vectors that 
transform under the action of a compact group \m{G} as 
\m{\V r_j\mapsto [\rho_{\Omega}]_g \V r_j}, then the corresponding \m{k}'th moment tensor, 
defined as in \rf{eq: moment tensor}, is 
(a) invariant with respect to permuting \m{\sseq{\V r}{m}} amongst themselves, (b) 
transforms according 
%Expressing the bulk properties of systems in terms of moments of differents orders, such as the above, 
%is a recurring theme in Physics, so it is natural to expect \m{\V r^{\otimes k}:=\V r\otimes\ldots\otimes \V r} 
%to make an appearance in \m{\Phi}. The above equations (which generalize to 
%any compact group, not just rotations) tell us that \m{\V r^{\otimes k}} transforms according 
to the tensor product representation %\m{\cbrN{\rho_\Omega^k}} defined 
\[\rho^{k}_\Omega(g):=[\rho_{\Omega}(g)]^{\otimes k}=
\underbrace{\rho_{\Omega}(g)\otimes \rho_{\Omega}(g)\otimes \ldots\otimes \rho_{\Omega}(g)}_{k\textrm{ times}}\]
with respect to the action of \m{G}. 
Moment tensors are widely used in different branches of Physics to describe the aggregate spatial 
properties of collections of particles or subsystems. 
Most recently, they were successfully used to 



At the same time, the state vector \m{\phi_i} transforms according to the representation \m{\rho_i}, 
so its \m{p}'th tensor product will transform according to \m{\rho_i^p}. 
Therefore, any combination of tensor powers of the form  
\[\V r_i^{\otimes k}\otimes \phi_i^{\otimes p}\]
is a potential building block of \m{\Phi}. 
With regard to symmetry in the ordering of the children, we can just use symmetric polynomials of 
order q. 

\begin{proposition}
Let \m{\neuron_{\ch_1},\ldots,\neuron_{\ch_c}} be the children of \m{\neuron_j} in a covariant neural model. 
Assume that \m{\phi_{\ch_i}} are in the same representation space \m{V} of \m{G} 
for each \m{i\tin\cbrN{\oneton{c}}}, and let \m{\Scal_q} be the \m{q}'th elementary symmetric polynomial. 
Then the vector 
\[\xi=\Scal_q(\V r_{\ch_1}^{\otimes k}\<\otimes \phi_{\ch_1}^{\otimes p},\,\ldots\:,
\V r_{\ch_c}^{\otimes k}\<\otimes \phi_{\ch_c}^{\otimes p})\] 
is symmetric with respect to permutations of \m{\cbrN{\ch_1,\ldots,\ch_c}}, and 
transforms according to the representation \m{\rho_{\Omega}^{qk}\otimes \rho_{V}^{qp}} according to the action 
of \m{G}. 
\end{proposition}
\bigskip

\noindent 
For simplicity, in the following we only consider the case \m{q=p=1}. Thus we have the following 
definition. 

\begin{definition}
The aggregation function in a \m{k}'th \df{order neural model of a Physical system} is of the form 
\[\Phi(\V r_{\ch_1},\ldots,\V r_{\ch_c},\phi_{\ch_1}\ldots,\phi_{\ch_c})=
\sigma\brBig {\Wcal\brBig{ \sum_{i=1}^{c} \V r_i^{\otimes k} \otimes \phi_i}},\]
where  \m{\V r_{\ch_{i}}=\x_{\ch_i}\<-\x_j}, and \m{\Wcal} is a learnable linear function. 
\end{definition}

\begin{theorem}
Let \m{\seqi{\rho}} be a complete set of inequivalent irreducible representations of \m{G}, and 
\[\rho_\Omega^k\otimes V=\bigoplus_{p} \bigoplus_{a=1}^{\kappa(p)} W_p\] 
the decomposition of \m{\rho_\Omega^k\otimes V} into a sum of corresponding representation spaces. 
Given any \m{\V v\tin \rho_\Omega^k\otimes V}, let \m{\Vv\tdown_{(p,a)}} be its projection 
to the corresponding subspace. Then the \m{k}'th order neural model is covariant in the sense of CM4 
if and only if \m{\Wcal} is of the form 
\[[\Wcal \Vv]_{p,a}=\sum_{b=1}^{\kappa(p)} [W_{p}]_{a,b}\, \Vv\tdown_{(p,b)}.\]
\end{theorem}


